Knowledge-augmented Risk Assessment (KaRA): a hybrid-intelligence framework for supporting knowledge-intensive risk assessment of prospect candidates

Evaluating the potential of a prospective candidate is a common task in multiple decision-making processes in different industries. We refer to a prospect as something or someone that could potentially produce positive results in a given context, e.g., an area where an oil company could find oil, a compound that, when synthesized, results in a material with required properties, and so on. In many contexts, assessing the Probability of Success (PoS) of prospects heavily depends on experts' knowledge, often leading to biased and inconsistent assessments. We have developed the framework named KARA (Knowledge-augmented Risk Assessment) to address these issues. It combines multiple AI techniques that consider SMEs (Subject Matter Experts) feedback on top of a structured domain knowledge-base to support risk assessment processes of prospect candidates in knowledge-intensive contexts.

==> tex/UseCase.tex <==
\section{Case Study}
\label{case-study}

\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.85\textwidth]{img/trap-methodology}
	\caption{Contextual questionnaire of characterization methodology for trap structure risk factor based on reference risk table found in \cite{milkov2015risk}.}
	\label{fig-trap-met}
\end{figure*}

\begin{table*}[htb]
	\centering
\tiny
\setlength{\tabcolsep}{0.003\linewidth}
\begin{tabular}{
	p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
	p{0.032\linewidth}
	p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
	p{0.032\linewidth}
	p{0.032\linewidth}
	p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
	p{0.032\linewidth}
	p{0.032\linewidth}
	p{0.032\linewidth}
	p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
	>{\columncolor[gray]{.8}}p{0.032\linewidth}
}\toprule
	\textbf{p} & 
	\multicolumn{2}{>{\cellcolor[gray]{.8}}p{0.070\linewidth}}{\textbf{Seismic Calibration}} & 
	\multicolumn{2}{p{0.064\linewidth}}{\textbf{Seismic Data Type}} & 
	\multicolumn{3}{>{\cellcolor[gray]{.8}}p{0.108\linewidth}}{\textbf{Seismic Density}} & 
	\multicolumn{3}{p{0.096\linewidth}}{\textbf{Seismic Data Visual Quality}} & 
	\multicolumn{3}{>{\cellcolor[gray]{.8}}p{0.108\linewidth}}{\textbf{Structure Interpretation}} & 
	\multicolumn{4}{p{0.128\linewidth}}{\textbf{Structure Complexity}} & 
	\multicolumn{3}{>{\cellcolor[gray]{.8}}p{0.108\linewidth}}{\textbf{Structural Relief}} \\ \hline
	%%
	& \rot{Yes} & \rot{No} & \rot{3D} & \rot{2D} & \rot{Dense} & \rot{Sparse} & \rot{Very Sparse} & \rot{Good} & \rot{Medium} & \rot{Bad} & \rot{Easy/reliable} & \rot{Uncertain} & \rot{Unreliable} & \rot{4-way} & \rot{3-way} & \rot{2-way} & \rot{Stratigraphic} & \rot{Low-relief} & \rot{Medium-relief \ } & \rot{High-relief} \\ \hline
	\textbf{A}  & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 \\
	\textbf{B}  & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 1 \\
	\textbf{C}  & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 \\
	\textbf{D}  & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 1 & 0 & 0 \\
	\textbf{E}  & 0 & 1 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 1 & 0 & 0 \\
	\bottomrule
\end{tabular}
\label{tab:prospect-charac-examples}
\caption{Prospect characterization examples for trap strucuture risk factor using one-hot encoding representation.}
\end{table*}

\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{img/LOK-Graph-all.pdf}
	\caption{All experts (global) LOK conflicts graph}
	\label{fig-global-lok-conflicts-graph}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{img/LOK-Graph-all-opt.pdf}
	\caption{Conflicts graph for global LOK consensus solution.}
	\label{fig-global-lok-consensus-graph}
\end{figure}



% POS A = 15% - LOK = 
% POS B = 95% - LOK =
% POS C = 50% - LOK =
% POS D = 50% - LOK =
% POS E = 0.05% - LOK = 

% 
% E -> A -> C -> D -> B

